Opportunistic Edge Computing: Concepts, Opportunities and Research Challenges

The growing need for low-latency access to computing resources has motivated the introduction of edge computing, where resources are strategically placed at the access networks. Unfortunately, edge computing infrastructures like fogs and cloudlets have limited scalability and may be prohibitively expensive to install given the vast edge of the Internet. In this paper, we present Opportunistic Edge Computing (OEC), a new computing paradigm that provides a framework to create scalable infrastructures at the edge using end-user contributed resources. One of the goals of OEC is to place resources where there is high demand for them by incentivizing people to share their resources. This paper defines the OEC paradigm and the involved stakeholders and puts forward a management framework to build, manage and monitor scalable edge infrastructures. It also highlights the key differences between the OEC computing models and the existing computing models and shed the light on early works on the topic. The paper also presents preliminary experimental results that highlight the benefits and the limitations of OEC compared to the regular cloud computing deployment and the Fog deployment. It finally summarizes key research directions pertaining to resource management in OEC environments.

==> related.tex <==

\section{Related Work}
\label{related}

Immense popularity of mobile computing has motivated several researchers to
investigate the opportunistic formation of cloud computing services to better
support mobile and ad hoc computing requirements of resource-intensive
applications. In this paper, we present a novel architecture that extends
opportunistic computing to the edge and identify important research problems
that need to be solved to implement OCC. In this section, we explain how the OCC
concept is different from previously proposed systems.

One of the systems that has many similarities to OCC is the
Collective Manager (CM) by S. Goyal~\cite{goyal_phd}. The CM is central broker
that aggregates volunteer resources and orchestrates their operation to deliver
predefined services such as content distribution and backup to the clients. End
users get paid in a virtual currency for contributing resources in a consistent
manner and can use the currency to use the services offered by the CM. Although
CM has resources at the edge because they are end-user contributed, edge
computing is not the goal of CM; instead, CM focuses on extracting quality of
service out of volunteer computing. CM has incentive management schemes that operate
with complete or incomplete information regarding the resource sharing activities
of the end users.
Several problems such as location-based
computation of incentives and edge network optimization for resource provisioning
highlighted by this paper are not considered by CM.

In~\cite{mascitti2014service}, Mascitti et al. created a system,
where mobile devices directly provide services to each
other without necessarily going through cloud-resident services.
Their algorithm takes into account both the mobility of the devices and
their computational capabilities to derive stochastic measures useful for
comparing the possible alternatives to satisfy a request for service.
The algorithm selects the best alternative for providing the service to a client
among the available services on other mobile devices.

In~\cite{6450900}, an
incentive mechanism for Opportunistic Cloud Computing Services (OCCS) was
proposed. They looked to motivate the donation of computing
resources to the resource pool within the system and also to ensure an effective
and efficient usage of the available computing resources. They used a game
theory-based approach and also showed that Nash equilibrium exists for the two game
models they dealt with; cooperative and non-cooperative games. They argued that
the OCCS network may suffer from problems like some users being selfish and only
want to use resources without having to contribute. Also, some users can waste
resources (knowingly or unknowingly) or agents external to the system trying to
cause denial of service.

The game model in~\cite{6450900} is as follows, a member joins a game by
donating, using or subscribing to a particular service. A user can participate
in as many games as possible. Games are independent and are allocated a time
frame. So, games are repeated based on the time slot. Players tend to maximize
their own profit in a non-cooperative game, while players try to maximize their
own profits and that of their collaborating partners in a cooperative game.

A similar model was proposed in \cite{Kuada2013}. A trust management scheme was
developed for Opportunistic Cloud Services (OCS). OCS involves organizations
contributing and using spare computing resources in form of cloud services. In
the system proposed, members package their spare computing resources and donate
them to the OCS platform (a centralized control platform). Trust is the level of
confidence of a service consumer that the outcome of a transaction with a
service provider will be satisfactory for it and vice versa. The trust level of
a service is defined as the priori probability that the request of the service
consumer will be met or will exceed the minimum satisfaction threshold at the
end of the transaction.

The OCS platform in \cite{Kuada2013} can serve as a
trust generator using these two basic approaches; the trusted third party-based
approach and reputation-based approach. The platform is focused majorly on the
applicability and usability properties. The main elements and operations of the
trust management system are: expectation (in the form of SLA), data monitoring,
data management, data analysis and decision making.

